See It All: Contextualized Late Aggregation for 3D Dense Captioning

3D dense captioning is a task to localize objects in a 3D scene and generate descriptive sentences for each object. Recent approaches in 3D dense captioning have adopted transformer encoder-decoder frameworks from object detection to build an end-to-end pipeline without hand-crafted components. However, these approaches struggle with contradicting objectives where a single query attention has to simultaneously view both the tightly localized object regions and contextual environment. To overcome this challenge, we introduce SIA (See-It-All), a transformer pipeline that engages in 3D dense captioning with a novel paradigm called late aggregation. SIA simultaneously decodes two sets of queries-context query and instance query. The instance query focuses on localization and object attribute descriptions, while the context query versatilely captures the region-of-interest of relationships between multiple objects or with the global scene, then aggregated afterwards (i.e., late aggregation) via simple distance-based measures. To further enhance the quality of contextualized caption generation, we design a novel aggregator to generate a fully informed caption based on the surrounding context, the global environment, and object instances. Extensive experiments on two of the most widely-used 3D dense captioning datasets demonstrate that our proposed method achieves a significant improvement over prior methods.

==> section/6_related_work.tex <==
\section{Related Work}
\label{sec:related_work}
\paragraph{Image Captioning.}
Image captioning is a fundamental task in visual-language generation that involves the automatically generating descriptive sentences for images. This task has attracted significant research interest due to its critical applications in assistive technology, content retrieval and multimedia systems. The primary goal is to improve 2D scene understanding \cite{hossain2019comprehensive}.

In the early stages of image captioning, the dominant techniques centered around template-based approaches \cite{farhadi2010every} that formed sentences based on predefined structures.
Concurrently, retrieval-based mechanisms \cite{wu2017automatic} were employed, where the most suitable sentence was selected from a repository of potential captions for a specific image.
However, with the advancement of deep learning in image captioning, there has been a marked shift towards the development and adoption of more sophisticated models \cite{ghandi2022deep}.

% \paragraph{Encoder-Decoder.}
% The development of deep learning in image captioning was marked by the adoption of the encoder-decoder framework.
% Convolutional Nerual Networks (CNNs) \cite{krizhevsky2012imagenet,he2016deep,huang2017densely} emerged as effective encoders, transforming visual content into compact feature vectors.
% These vectors were subsequently processed by Recurrent Neural Networks (RNNs) \cite{hochreiter1997long,cho2014learning} to produce descriptive captions.
% The inclusion of object detectors aimed to improve feature extraction, and attention mechanisms especially as demonstrated by the "Show, Attend and Tell" method \cite{xu2015show}, allowed models to selectively focus on critical regions within images \cite{cornia2020meshed}.
% The integration of graph neural networks further enhanced the contextual understanding of images, as exemplified by notable research like exploration of auto-encoding scene graphs \cite{yang2019auto}.

\paragraph{Taling through Transformers.}
Moreover, the introduction of transformers \cite{vaswani2017attention,cornia2020meshed,herdade2019image} marked a transformative phase in the field. Initially developed for a language processing, this architecture achieved considerable success in image captioning due to its outstanding ability to understand and generate sequences. When combined with Vision-Language Pretrained (VLP) models, transformer demonstrated exceptional potential in image captioning. ConZIC \cite{zeng2023conzic} emerged as a crucial model in this area, drawing on the strengths of both BERT \cite{devlin2018bert} and CLIP \cite{radford2021learning} to enable controllable zero-shot image captioning, and thereby establishing a novel benchmark in generation speed and efficiency.
 
\paragraph{3D Dense Captioning.}
3D dense captioning is a task that aims to achieve object level 3D scene understanding by generating natural language descriptions for objects in 3D scenes through the analysis of 3D visual data \cite{chen2021scan2cap}.
The existing approaches in the field of 3D dense captioning can be categorized based on research focus~\cite{yu2023comprehensive}.





% \cite{chen2021scan2cap}, \cite{chen2020scanrefer}, \cite{achlioptas2020referit3d} \cite{chen2022d3net}, \cite{yuan2022xtrans2cap}, \cite{wang2022spacap3d}, \cite{jiao2022more}, \cite{cai20223djcg}, \cite{chen2023vote2capdetr}, \cite{zhong2022contextual}
% \hs{ScanRefer, ReferIt3D, Scan2Cap, D3Net, X-Trans2Cap, SpaCap3D, MORE, 3DJCG, CM3D, Vote2Cap-DETR}

==> section/responsible.tex <==
- Add analysis of captions generated using object features vs aggregated, context aware features

- Experiment ablations on the design choices and hyper-parameters

- Experiments on expansion of ROI radius

- Clarify details on how final caption is generated and how the loss functions are used 

- Provide details of baselines

- Improve terminology. Reviewer R-YvSK noted that the term "caption-centric dense captioning" is confusing and recommends the the term "context-aware dense captioning". The AE agrees that it is unclear what "caption-centric" refers to and that "context-aware" is more clear.

- Add references and discussion to suggested dense image captioning methods

- Improvements to figures and table captions

- Editing pass to fix typos


==> tables/ablation_key_components.tex <==
\begin{table*}[t]
   \centering
   \resizebox{\textwidth}{!}{%
     \begin{tabular}{cc@{\hspace{30pt}}|cccccc|cccccc}
     \toprule
     \multirow{1}{*}{} & \multicolumn{1}{c}{} & \multicolumn{6}{c}{IoU=$0.25$} & \multicolumn{6}{c}{IoU=$0.50$} \\
     \cmidrule(lr){3-8} \cmidrule(lr){9-14}
     \multirow{1}{*}{Model} & \multicolumn{1}{c}{Training} & \multicolumn{1}{c}{C$\uparrow$} & \multicolumn{1}{c}{B-4$\uparrow$} & \multicolumn{1}{c}{M$\uparrow$} & \multicolumn{1}{c}{R$\uparrow$} & \multicolumn{1}{c}{mAP$\uparrow$} & \multicolumn{1}{c}{AR$\uparrow$} & \multicolumn{1}{c}{C$\uparrow$} & \multicolumn{1}{c}{B-4$\uparrow$} & \multicolumn{1}{c}{M$\uparrow$} & \multicolumn{1}{c}{R$\uparrow$} & \multicolumn{1}{c}{mAP$\uparrow$} & \multicolumn{1}{c}{AR$\uparrow$}\\
     \midrule
     \midrule

     %\multirow{1}{*}{3DJCG} & \multicolumn{1}{c}{} 
     %& \multicolumn{1}{c}{60.86} & \multicolumn{1}{c}{39.67} & \multicolumn{1}{c}{27.45} & \multicolumn{1}{c}{59.02} 
     %& \multicolumn{1}{c}{47.68} & \multicolumn{1}{c}{31.53} & \multicolumn{1}{c}{24.28} & \multicolumn{1}{c}{51.80} \\

     %\multirow{1}{*}{3D-VLP} & \multicolumn{1}{c}{} 
     %& \multicolumn{1}{c}{64.09} & \multicolumn{1}{c}{39.84} & \multicolumn{1}{c}{27.65} & \multicolumn{1}{c}{58.78}
     %& \multicolumn{1}{c}{50.02} & \multicolumn{1}{c}{31.87} & \multicolumn{1}{c}{24.53} & \multicolumn{1}{c}{51.17} \\

     \multirow{1}{*}{Vote2Cap-DETR} & \multicolumn{1}{c}{} 
     & \multicolumn{1}{c}{71.45} & \multicolumn{1}{c}{39.34} & \multicolumn{1}{c}{28.25} & \multicolumn{1}{c}{59.33} & \multicolumn{1}{c}{65.05} & \multicolumn{1}{c}{87.40}
     & \multicolumn{1}{c}{61.81} & \multicolumn{1}{c}{34.46} & \multicolumn{1}{c}{26.22} & \multicolumn{1}{c}{54.40} & \multicolumn{1}{c}{45.56} & \multicolumn{1}{c}{67.77} \\

     \multirow{1}{*}{SIA with $V^o$} & \multicolumn{1}{c}{} 
     & \multicolumn{1}{c}{74.37} & \multicolumn{1}{c}{41.55} & \multicolumn{1}{c}{28.17} & \multicolumn{1}{c}{60.49} & \multicolumn{1}{c}{65.66} & \multicolumn{1}{c}{87.08}
     & \multicolumn{1}{c}{64.75} & \multicolumn{1}{c}{36.76} & \multicolumn{1}{c}{26.23} & \multicolumn{1}{c}{55.63} & \multicolumn{1}{c}{46.15} & \multicolumn{1}{c}{65.85} \\

     \multirow{1}{*}{SIA with $V^o$, $V^c$} & \multicolumn{1}{c}{MLE} 
     & \multicolumn{1}{c}{77.24} & \multicolumn{1}{c}{42.64} & \multicolumn{1}{c}{28.27} & \multicolumn{1}{c}{59.89} & \multicolumn{1}{c}{69.26} & \multicolumn{1}{c}{88.04}
     & \multicolumn{1}{c}{\textbf{73.38}} & \multicolumn{1}{c}{37.92} & \multicolumn{1}{c}{26.14} & \multicolumn{1}{c}{54.74} & \multicolumn{1}{c}{48.74} & \multicolumn{1}{c}{67.04} \\

     \multirow{1}{*}{\textbf{SIA with $V^o$, $V^c$, $V^a$ (Ours)}} & \multicolumn{1}{c}{} 
     & \multicolumn{1}{c}{\textbf{78.68}} & \multicolumn{1}{c}{\textbf{43.25}} & \multicolumn{1}{c}{\textbf{29.21}} & \multicolumn{1}{c}{\textbf{63.06}} & \multicolumn{1}{c}{\textbf{72.20}} & \multicolumn{1}{c}{\textbf{88.09}}
     & \multicolumn{1}{c}{73.22} & \multicolumn{1}{c}{\textbf{40.91}} & \multicolumn{1}{c}{\textbf{28.19}} & \multicolumn{1}{c}{\textbf{60.46}} & \multicolumn{1}{c}{\textbf{49.69}} & \multicolumn{1}{c}{\textbf{69.08}} \\
     
     \midrule

     %\multirow{1}{*}{$\chi$-Tran2Cap} & \multicolumn{1}{c}{} 
     %& \multicolumn{1}{c}{58.81} & \multicolumn{1}{c}{34.17} & \multicolumn{1}{c}{25.81} & \multicolumn{1}{c}{54.10} 
     %& \multicolumn{1}{c}{41.52} & \multicolumn{1}{c}{23.83} & \multicolumn{1}{c}{21.90} & \multicolumn{1}{c}{44.97} \\

     \multirow{1}{*}{Vote2Cap-DETR} & \multicolumn{1}{c}{} 
     & \multicolumn{1}{c}{84.15} & \multicolumn{1}{c}{42.51} & \multicolumn{1}{c}{28.47} & \multicolumn{1}{c}{59.26} & \multicolumn{1}{c}{65.05} & \multicolumn{1}{c}{87.40}
     & \multicolumn{1}{c}{73.77} & \multicolumn{1}{c}{38.21} & \multicolumn{1}{c}{26.64} & \multicolumn{1}{c}{54.71} & \multicolumn{1}{c}{45.56} & \multicolumn{1}{c}{67.77} \\

     \multirow{1}{*}{SIA with $V^o$} & \multicolumn{1}{c}{} 
     & \multicolumn{1}{c}{85.10} & \multicolumn{1}{c}{44.06} & \multicolumn{1}{c}{28.30} & \multicolumn{1}{c}{60.44} & \multicolumn{1}{c}{65.66} & \multicolumn{1}{c}{87.08}
     & \multicolumn{1}{c}{73.80} & \multicolumn{1}{c}{39.06} & \multicolumn{1}{c}{26.33} & \multicolumn{1}{c}{55.50} & \multicolumn{1}{c}{46.15} & \multicolumn{1}{c}{65.85} \\

     \multirow{1}{*}{SIA with $V^o, V^c$} & \multicolumn{1}{c}{SCST} 
     & \multicolumn{1}{c}{89.34} & \multicolumn{1}{c}{43.30} & \multicolumn{1}{c}{28.70} & \multicolumn{1}{c}{60.33} & \multicolumn{1}{c}{69.26} & \multicolumn{1}{c}{88.04}
     & \multicolumn{1}{c}{81.45} & \multicolumn{1}{c}{41.19} & \multicolumn{1}{c}{26.22} & \multicolumn{1}{c}{55.34} & \multicolumn{1}{c}{48.74} & \multicolumn{1}{c}{67.04} \\

     \multirow{1}{*}{\textbf{SIA with $V^o, V^c, V^a$ (Ours)}} & \multicolumn{1}{c}{}
     & \multicolumn{1}{c}{\textbf{89.72}} & \multicolumn{1}{c}{\textbf{44.56}} & \multicolumn{1}{c}{\textbf{28.96}} & \multicolumn{1}{c}{\textbf{62.13}} & \multicolumn{1}{c}{\textbf{72.20}} & \multicolumn{1}{c}{\textbf{88.09}}
     & \multicolumn{1}{c}{\textbf{83.14}} & \multicolumn{1}{c}{\textbf{42.17}} & \multicolumn{1}{c}{\textbf{27.92}} & \multicolumn{1}{c}{\textbf{59.44}} & \multicolumn{1}{c}{\textbf{49.69}} & \multicolumn{1}{c}{\textbf{69.08}} \\

     \bottomrule
     \end{tabular}
     }
 \caption{Ablation study on the ScanRefer~\cite{chen2020scanrefer} dataset. The core components of our model: instance query feature $V^o$, context query feature $V^c$, and TGI-Aggregator feature $V^a$, respectively.}
 \label{tab:ablation_key_components}
 \end{table*} 

==> tables/analysis_radius.tex <==
\begin{table*}
   \centering
   \resizebox{\textwidth}{!}{%
     \begin{tabular}{c|cccc}
     \toprule
     \multirow{1}{*}{} & \multicolumn{1}{c}{C@$0.5\uparrow$} & \multicolumn{1}{c}{B-4@$0.5\uparrow$} & \multicolumn{1}{c}{M@$0.5\uparrow$} & \multicolumn{1}{c}{R@$0.5\uparrow$} \\
     \midrule
     \midrule

    \multirow{1}{*}{Instance Query Generator with radius=$0.3$} & \multicolumn{1}{c}{64.75} & \multicolumn{1}{c}{36.76} & \multicolumn{1}{c}{26.23} & \multicolumn{1}{c}{55.63} \\
     
    \multirow{1}{*}{Instance Query Generator with radius=$0.8$} & \multicolumn{1}{c}{56.62} & \multicolumn{1}{c}{34.77} & \multicolumn{1}{c}{24.84} & \multicolumn{1}{c}{52.03} \\   
    
    \midrule
    
    \multirow{1}{*}{Instance Query Generator with radius=$0.3$ \& Context Query Generator with radius=$0.8$} & \multicolumn{1}{c}{70.73} & \multicolumn{1}{c}{39.13} & \multicolumn{1}{c}{27.89} & \multicolumn{1}{c}{56.33} \\ 
    
    \multirow{1}{*}{Instance Query Generator with radius=$0.3$ \& Context Query Generator with radius=$1.2$} & \multicolumn{1}{c}{\textbf{73.22}} & \multicolumn{1}{c}{\textbf{40.91}} & \multicolumn{1}{c}{\textbf{28.19}} & \multicolumn{1}{c}{\textbf{60.46}} \\
    
     \bottomrule
     \end{tabular}
     }
 \caption{Experimental results of expanding ROI radius in ScanRefer~\cite{chen2020scanrefer}.}
 \label{tab:analysis_radius}
 \end{table*} 

==> tables/global_caption.tex <==
\begin{table}
   \centering
   \resizebox{\linewidth}{!}{%
     \begin{tabular}{c|cccc}
     \toprule
     \multirow{1}{*}{object} & \multicolumn{1}{c}{C@$0.5\uparrow$} & \multicolumn{1}{c}{B-4@$0.5\uparrow$} & \multicolumn{1}{c}{M@$0.5\uparrow$} & \multicolumn{1}{c}{R@$0.5\uparrow$} \\
     \midrule
     \midrule

     \multirow{1}{*}{Contexts $V^c$} & \multicolumn{1}{c}{72.82} & \multicolumn{1}{c}{38.46} & \multicolumn{1}{c}{26.76} & \multicolumn{1}{c}{56.71} \\
          
     \multirow{1}{*}{Single Instance $V^o_i$ \& Contexts $V^c$} & \multicolumn{1}{c}{72.89} & \multicolumn{1}{c}{38.21} & \multicolumn{1}{c}{27.04} & \multicolumn{1}{c}{57.33} \\

     \multirow{1}{*}{\textbf{Instances $V^o$ \& Contexts $V^c$}} & \multicolumn{1}{c}{\textbf{73.22}} & \multicolumn{1}{c}{\textbf{40.91}} & \multicolumn{1}{c}{\textbf{28.19}} & \multicolumn{1}{c}{\textbf{60.46}} \\
     
     \bottomrule
     \end{tabular}
     }
 \caption{global caption}
 \label{tab:global_caption}
 \end{table} 
